Parallel Loop Transformer for Efficient Test-Time Computation Scaling

Large Language Models (LLMs) are powerful but often too slow and costly for real-world use during inference. Looped transformers save on parameters by reusing the same weights for multiple computational steps, or "loops." However, this approach has a major flaw: the loops run one after another, causing inference latency and memory requirements to increase with each added loop. This makes them impractical for fast applications. To solve this problem, we introduce the Parallel Loop Transformer (PLT). PLT is a new architecture that delivers the performance benefits of a deep, looped model but with the low latency of a standard, non-looped model. PLT works using two key techniques. First, Cross-Loop Parallelism (CLP) breaks the sequential dependency by computing different loops for different tokens at the same time, all within a single pass. Second, to prevent memory costs from growing, we use an Efficient Representation Enhancement strategy. This method shares the memory (KV cache) from the first loop with all other loops. It then uses a Gated Sliding-Window Attention (G-SWA) to combine this shared global information with local information, maintaining high accuracy. Our experiments show that PLT achieves the high accuracy of a traditional looped model but with almost no extra latency or memory cost compared to a standard transformer.

==> sections/approach_old_backup.tex <==
\section{Approach}
\begin{figure}[tbp]
    \centering
    % 第一个子图 (a)
    \begin{subfigure}[b]{0.44\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/phdv2_figures/figure1_activation_origin_loop.drawio.png}
        \caption{Inference pipeline in original loop Transformer}
        \label{fig:loop_trans}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.44\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/phdv2_figures/figure1_activation_ours_loop.drawio.png}
        \caption{Inference pipeline in our proposed \method.}
        \label{fig:our_infer}
    \end{subfigure}
    
    \caption{Activation dependency in original loop transformer and our modification. The left figure presents the original activation dependency in loop Transformers, where each loop in each token should be computed in serial manner. 
    The right figure presents our modification in \method. The transformer loops within the same dashed box can be computed in parallel, leading to extremely better inference efficiency.}
    \label{fig-1: PHD-v2-motivation}
\end{figure}

\subsection{Main Architecture}


\subsection{Notations} \label{sec:notation}

We set up the notations in this section. Under the discussion framework of Loop Transformers, assume a training sample $T$ contains $n$ tokens $\{T_1, T_2, ..., T_t, ..., T_n\}$. We are using a looped transformer of $L$ loops. Denote $i_t^{loop-j}$ and $h_t^{loop-j}$ as the input/output of $j^{th}$ transformer loop respectively, the original activation dependency Logic of Loop Transformer can be written in the following formulas including Equation~\ref{form1},~\ref{form2} and ~\ref{form3}.

\begin{flalign} 
h_t^{loop-(l+1)} &= f_{loop-l}(i_t^{loop-(l)}) \label{form1} \\
i_t^{loop-(l+1)} &= h_t^{loop-(l)} \label{form2} \\
t_{i+1} &= f_{lm-head}(h_t^{loop-(L)}) \label{form3}
\end{flalign}

From the formulas presented above, the main drawback of looped-transformers is that the loops and tokens can only be calculated in the serial manner, which is also presented in Figure~\ref{fig:loop_trans}. Specifically, the latter loops depends on the output from the previous loops, while the first loop in each token depends on the last loop of previous tokens.



% where the hidden representation of each token can be represented as $\mathbf{h} = \{h_1, h_2, ..., h_t\}$, and the hidden dimension of each token is $d$. 

% Let $M_{mn}$ be the attention mask between $x_m$ and $x_n$, the original self-attention within sample $x$ can be written as follows:

% \begin{equation}
%     \text{Self-Attention}(\mathbf{h}) = \text{softmax}\left(\frac{(W_q \mathbf{h}) (W_k \mathbf{h})^\top \otimes M}{\sqrt{d}}\right) (W_v \mathbf{h}).
% \end{equation}

% Taking loop transformer into consideration, assuming we are using a loop number of $L$, we denote the activation of $x_i$ after loop $l$ as $x_i^l$. Denote the parameter of loop Transformer as $\theta$, then we have $x_i^l = f_\theta(x_{\leq i}^{l-1})$. 


\subsection{Displaced Parallelism across different tokens}   \label{sec:strectch_activation}


\begin{figure}[tbp]
    \centering
    % 第一个子图 (a)
    \centering
    \includegraphics[width=0.8\textwidth]{figures/phdv2_figures/training_share_kv_cache.drawio.png}
    \caption{The training pipeline of our proposed \method. All the loops share the KV cache produced by Loop-1. Boxes with the same color presents how the input tokens get through all the transformer loops and predict the target token. Specifically, Token $T_1$ go through three transformer loops to predict token $T_4$, which is also presented in Figure~\ref{fig:our_infer}. The training process is parallel in the token latitude, while serial in the loop latitude.}
    \label{fig:loop_train_sharekv}
\end{figure}


% \begin{flalign} \label{loop_form} 
% h_i^{loop-(l+1)} &= f_{loop-l}(h_i^{loop-(l)})\\
% t_{i+1} &= f_{lm-head}(h_i^{loop-(L)})
% \end{flalign}


% Specifically, the calculation of $x_i^{l+1}$ depends on $x_i^{l}$, meaning these transformer blocks can only be calculated in the serial manner. 

We propose displaced Parallelism across different loops in different tokens. \textbf{Specifically, we overlap the calculation of latter loops in previous tokens with former loops in current tokens.} We present the inference pipeline of our \method~in Figure~\ref{fig:our_infer} to compare with the inference pipeline of original loop transformers in Figure~\ref{fig:loop_trans}.

To address the concern that loop transformers are trained in the serial manner while our \method propose to inference Loop Transformer in parallel, we would like to clarify that the training and inference are consistent, which is also the core design of our paper. 

Specifically, there exists two serial latitudes in the training of Loop Transformers, including the loop latitude and token latitude, making it possible for us to parallelize different latitude in training and inference. Shown in Figure~\ref{fig:loop_train_sharekv}, during training, we compute serially in the loop latitude, and parallel in the token latitude which is supported by FlashAttention~\cite{dao2023flashattention,dao2024flashattention2}. 
Shown in Figure~\ref{fig:parallel_decode}, during inference, we compute serially in the token latitude, while parallel in the loop latitude.

\paragraph{Training formula} Denote $\mathbf{H}_{1...t}^{loop-l}=[h_1^{loop-l}, h_2^{loop-l}, ..., h_t^{loop-l}]$ and $\mathbf{I}_{1...t}^{loop-l}=[i_1^{loop-l}, i_2^{loop-l}, ..., i_t^{loop-l}]$. In training, the formula can be written in Equation~\ref{form4}, ~\ref{form5}, ~\ref{form6} and~\ref{form7}, which is also presented in Figure~\ref{fig:loop_train_sharekv}.

\begin{flalign}
\mathbf{H}_{m...n}^{loop-(l+1)} &= f_{loop-l}(\mathbf{I}_{(m)...(n)}^{loop-(l+1)}) \label{form4} \\
\mathbf{I}_{m...n}^{loop-(l+1)} &= f_{connector}(\mathbf{H}_{(m-1)...(n-1)}^{loop-(l+1)}, \mathbf{T}_{m...n}) \label{form5} \\
\mathbf{H}_{t<0}^{loop-(l)} &= \mathbf{0} \label{form6} \\
\mathbf{T}_{m...n} &= f_{lm-head}(\mathbf{H}_{(m-1)...(n-1)}^{loop-L}) \label{form7}
\end{flalign}

\paragraph{Inference formula} In inference, since the parallelism contains two latitudes at the same time (token level and loop level), for clarity, we only take $L=3$ as an example to write the formula. Assume we have already decoded token $T_{t+2}$, Equation~\ref{form8},~\ref{form9} and~\ref{form10} presents how we decode $T_{t+3}$ in parallel. The parallelized decoding procedure is also presented in Figure~\ref{fig:parallel_decode}.


\begin{flalign}
    [i_{t}^{loop-2}, i_{t+1}^{loop-1}, i_{t+2}^{loop-0}] &= f_{connector}([h_{t}^{loop-2}, h_{t+1}^{loop-1}, 0], [T_{t+2}, T_{t+2}, T_{t+2}]) \label{form8} \\
    [h_{t}^{loop-3}, h_{t+1}^{loop-2}, h_{t+2}^{loop-1}] &= f_{loop}([i_{t}^{loop-2}, i_{t+1}^{loop-1}, i_{t+2}^{loop-0}]) \label{form9} \\
    T_{t+3} &= f_{lm-head}(h_{t}^{loop-3}) \label{form10}
\end{flalign}



% To enable fast inference speed and low prefilling cost, we further introduce two core techniques in our design. 

\paragraph{KV Cache Sharing across different loops} To maintain the same memory access during inference, we propose KV sharing across different loops. Specifically, all the latter loops share the totally same KV cache with the first transformer loop. During inference, we forward different tokens in different loops in parallel. The KV cache sharing strategy enables us with the feasibility to forward parallel loops with the same memory access since all these loops use the same copy of KV cache.

\paragraph{Sliding window attention for different loops} To increase the final performance without substantially increasing the memory access, we propose to maintain sliding window attention for different loops except for loop 1. In this way, we have two attention outputs in the latter transformer loops. We use a simple gating mechanism to fuse these two attention outputs. The following formulas present our gating method, with the input hidden representation denoted as $h$, the shared key states and value states in loop 1 as $k_{share}$ and $v_{share}$, and the window size $w$.
\begin{align}
    q, k, v &= W_Q^Th, W_K^Th,W_V^Th \label{eq:qkv_proj}\\
    o_{full} &= Attn(q, k_{share}, v_{share}) \label{eq:full_attn} \\
    o_{swa} &= Attn(q, k[-w:], v[-w:]) \label{eq: swa} \\
    gate_{o} &= f_{gate-mlp}(q) \label{eq: gate} \\
    o_{final} &= (1-gate_{o}) * o_{full} + gate_o * o_{swa} \label{eq: final}   
\end{align}



% \paragraph{Chunk-level Sliding Window Attention} Totally sharing the KV cache might leads to performance degradation, we further introduce chunk-level sliding window attention to improve the performance of latter loops with negligible memory-access overhead and prefilling overhead. 

% Figure~\ref{fig:chunk_slideing_window} presents our chunk-wise sliding window attention strategy. Inspired by xxx, the local window usually preserves the most of the information while introducing minimum memory access overhead during inference. However, vanilla sliding window attention leads to prefilling overhead, where we need to prefill $L\times$. We further introduce chunk-wise sliding window attention to enable faster prefilling, where we only need to prefill the last chunk for additional $L-1$ times.

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figures/phdv2_figures/figure_3_decode_parallel.drawio.png}
    \caption{Parallelized forward of \method in decoding $T_{t+2}$ and $T_{t+3}$ in a Loop Transformer of $L=3$. We maintain $L=3$ activations in parallel, where in the next decoding step, we combine them with the newly input word embedding, and forward them in parallel, with each activation updated to the next loop. The training process is parallel in the token latitude, while serial in the loop latitude. The inference process is serial in the token latitude, while parallel in different loops across different tokens.}
    \label{fig:parallel_decode}
\end{figure}


\subsection{Inference Efficiency Analysis} \label{sec:train_and_decode}


% \paragraph{Prefilling Efficiency}

% Our proposed \method introduce high efficiency in prefilling. Since we use KV-cache sharing strategy, all the transformer loops shares exactly the same KV-cache in Loop-1, meaning that we only need to prefill the first transformer loop, leading to extreme prefilling efficiency.

% \paragraph{Decoding Efficiency}
As show in Figure~\ref{fig:parallel_decode}, different from vanilla transformers that only decodes one token at each step, in \method, we need to maintain $L$ activations in parallel. The forward of these $L$ activations share exactly the same model parameters and global kv cache, except for a sliding window KV cache of length $w$. Given that the loop number $L$ is much smaller than the model dimension and sequence length and the window $w$ is also much smaller than sequence length $l$, in the parallel forward of these $L$ activations, the parallelism introduces negligible increase of memory access, while only $L$ times computation overhead. Under serving scenarios that suffers from severe memory-access bottleneck, the parallel computation introduces negligible latency overhead.



==> sections/exp_tables_new/ablation_phdv1_v2.tex <==
\begin{table}[tp]
    \centering
    \small
    \setlength{\tabcolsep}{7pt}
    \caption{Scaling ability w.r.t. the number of parallelized loop transformers on OLMo.}
    \begin{tabular}{l|c|ccccccc|c}
    \toprule
    & Loss & MMLU & Hella. & ARC-C & ARC-E & PIQA & Wino. & Comm. & Avg. \\
    \midrule
        Vanilla Dense& 2.759 & 31.7 & 52.2 & 29.9 & 63.1 & 71.9 & 56.8 & 41.0 & 49.5 \\
        
        \ \ +\textit{\method-2} & 2.706 & 32.5 & 55.3 & 32.4 & 63.2 & 72.5 & \textbf{58.0} & \textbf{41.0} & 50.7 \\
        \ \ +\textit{\method-3} & \textbf{2.684} & \textbf{33.5} & \textbf{56.9} & \textbf{33.2} & \textbf{65.1} & \textbf{72.5} & 56.9 & 40.3 & \textbf{51.2} \\
        % \textit{\method-5} & 2.673 & 33.0 & 58.2 & 35.4 & 66.1 & 73.7 & 57.5 & 42.9 & 52.4 \\

        % \midrule
        % Vanilla MoE& 2.476 & 35.1 & 61.2 & 33.4 & 64.7 & 74.9 & 59.7 & 42.5 & 53.1 \\
        
        % \ \ +\textit{\method-2} & 2.430 & 35.9 & 64.5 & \textbf{40.8} & \textbf{71.9 }& 75.8 & 62.2 & 46.4 & 56.8 \\
        % \ \ +\textit{\method-3} & \textbf{2.409} & \textbf{36.4} & \textbf{66.3} & 38.8 & 71.8 & \textbf{77.1} & \textbf{63.0} & \textbf{48.1} & \textbf{57.4} \\
        % \textit{PHD-v2-5} & 2.681 & 34.0 & 57.6 & 33.7 & 67.8 & 59.6 & 72.3 & 46.5 & 53.1 \\
    \bottomrule
    \end{tabular}
    \label{tab:scale_decode_token}
\end{table}


